Assessing Neural Referential Form Selectors on a Realistic Multilingual Dataset

Previous work on Neural Referring Expression Generation (REG) all uses WebNLG, an English dataset that has been shown to reflect a very limited range of referring expression (RE) use. To tackle this issue, we build a dataset based on the OntoNotes corpus that contains a broader range of RE use in both English and Chinese (a language that uses zero pronouns). We build neural Referential Form Selection (RFS) models accordingly, assess them on the dataset and conduct probing experiments. The experiments suggest that, compared to WebNLG, OntoNotes is better for assessing REG/RFS models. We compare English and Chinese RFS and confirm that, in line with linguistic theories, Chinese RFS depends more on discourse context than English.

==> table/en_results_underscores.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{4-way} & \multicolumn{3}{c}{3-way} & \multicolumn{3}{c}{2-way} \\\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
Model & P & R & F & P & R & F & P & R & F  \\ \midrule
\texttt{c-RNN}  & 50.77 & 45.89 & 46.38 & \underline{60.83} & 59.56 & \underline{59.94} & 73.33 & \underline{72.58} & \underline{72.84} \\
\texttt{ +Glove} & \underline{53.47} & \textbf{49.49} & \textbf{50.44} & \textbf{61.72} & \textbf{60.66} & \textbf{60.98} & \textbf{75.06} & \textbf{73.96} & \textbf{74.32} \\
\texttt{ConATT} & 52.32 & 45.88 & 46.89 & 59.66 & 58.71 & 59.08 & 71.86 & 71.38 & 71.56 \\
\texttt{ +Glove} & \textbf{54.55} & \underline{47.56} & \underline{48.14} & 59.75 & \underline{60.05} & 59.85 & \underline{73.84} & 72.32 & 72.66 \\
\bottomrule
\end{tabular}
\caption{Evaluation results of RFS systems on \ontonotesen with general entity tags.}
\label{tab:en_cls_result_underscore}
\end{table*}

==> table/engmeanmodel.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Fri Mar 11 19:57:43 2022
\begin{table}[ht]
\centering
\begin{tabular}{lcccc}
  \toprule
Models & Mean & Std.Dev & Min & Max \\ 
  \midrule
  \texttt{XGBoost} & 64.66 & 14.73 & 49.12 & 78.42 \\
  \texttt{c-RNN} & 68.88 & 6.67 & 62.38 & 75.70 \\ 
  \texttt{ +Glove} & 70.41 & 6.07 & 64.56 & 76.67 \\ 
  \texttt{ +BERT} & 71.46 & 9.48 & 61.89 & 80.85 \\
\texttt{ConATT} & 66.93 & 5.86 & 61.58 & 73.19 \\ 
 \texttt{ +Glove} & 68.09 & 6.19 & 62.51 & 74.75 \\ 
   
  
 
   \bottomrule
\end{tabular}
\caption{Mean macro-averaged F1 scores of the \ontonotesen models across all classifications.} 
\label{tab:engmeanmodel}
\end{table}


==> table/zhmeanmodel.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Fri Mar 11 18:39:45 2022
\begin{table}[ht]
\centering
\begin{tabular}{lcccc}
  \toprule
Models & Mean & Std.Dev & Min & Max \\ 
  \midrule
  \texttt{XGBoost} & 47.88 & 12.73 & 34.59 & 63.67 \\
  \texttt{c-RNN} & 55.77 & 6.31 & 49.62 & 64.59 \\ 
  \texttt{ +SGNS} & 58.14 & 6.12 & 51.56 & 66.37 \\
  \texttt{ +BERT} & 69.19 & 4.85 & 63.85 & 75.59 \\ 
  \texttt{ConATT} & 52.83 & 3.95 & 49.25 & 58.28 \\ 
  \texttt{ +SGNS} & 55.96 & 4.51 & 53.09 & 62.69 \\ 
  
   
   \bottomrule
\end{tabular}
\caption{Mean macro-averaged F1 scores of the \ontonoteszh models across all classifications.} 
\label{tab:zhmeanmodel}
\end{table}

